Conformal Predictions under Markovian Data

We study the split Conformal Prediction method when applied to Markovian data. We quantify the gap in terms of coverage induced by the correlations in the data (compared to exchangeable data). This gap strongly depends on the mixing properties of the underlying Markov chain, and we prove that it typically scales as $\sqrt{t_\mathrm{mix}\ln(n)/n}$ (where $t_\mathrm{mix}$ is the mixing time of the chain). We also derive upper bounds on the impact of the correlations on the size of the prediction set. Finally we present $K$-split CP, a method that consists in thinning the calibration dataset and that adapts to the mixing properties of the chain. Its coverage gap is reduced to $t_\mathrm{mix}/(n\ln(n))$ without really affecting the size of the prediction set. We finally test our algorithms on synthetic and real-world datasets.

==> 5.corrected_cp.tex <==
% \subsection{Estimation of $\gamma$}

% The lower bound on coverage given above depends on $t_\textrm{mix}$ which in general is unknown. However, it can estimated using the training dataset. We require the following assumption.

% \textbf{Assumption} The Markov chain is in a finite state space $\mathcal{X}$ and is reversible (in addition of being aperiodic and irreductible). In this case, the mixing time can be upper bounded by the spectral gap

% $$t_\textrm{mix}\leq \frac{1}{1-\lambda}\ln(\frac{4}{\pi^*}) $$

% where $\pi^*=\min_\mathcal{X} \pi$. $\lambda=\max(\lambda_2, |\lambda_{|\mathcal{X}|}|)$ where $1>\lambda_2\geq...\geq\lambda_{|\mathcal{X}|}\geq -1$ are the eigenvalues of $P$. 

% We also know that it implies that the chain is uniformly ergodic with constants $(C,\lambda)$ hence 

% $$\frac{1}{n}\sum_{i=1}^n||\nu_0P^{N+i}-\pi||_{TV}\leq C \frac{\lambda^{N+1}(1-\lambda^{n+1})}{n(1-\lambda)}$$

% Therefore in the asymptotic regime we have 

%     $$\gamma\sim \sqrt{t_\mathrm{mix}\frac{\ln n}{n}} \leq \sqrt{\frac{\ln n}{n(1-\lambda)}} $$

% as the last two terms due to geometric ergodicity are negligible when $n\rightarrow\infty$.

% \begin{theorem}[\cite{hsu2015mixing}]
%     Let $\hat{\lambda}$ be the estimator of $\lambda$, calculated on a separate trajectory of size $N$. Then for any $\delta\in[0,1]$

% $$\mathbb{P}_{D_\textrm{tr}}\big(|\hat{\lambda}-\lambda| \leq \hat{w}(N,\delta)\big) \geq 1-\delta$$

% where $\hat{w}(N,\delta)$ can be empirically calculated and has almost sure asymptotic rate of convergence

% % \begin{align*}
% %     \hat{w}(N,\delta)=\min\{ &O_N(\sqrt{\frac{\ln \frac{|\mathcal{X}|}{\delta}\ln N}{\pi^*(1-\lambda) N}}), \\
% %     &O_N(\frac{|\mathcal{X}|\min(|\mathcal{X}|,\ln \frac{1}{\pi^*})}{\pi^*(1-\lambda)}\sqrt{\frac{\ln\ln N}{\pi^*N}} )\}   
% % \end{align*}

% $$\hat{w}(N,\delta)=O_N(\sqrt{\frac{\ln \frac{|\mathcal{X}|}{\delta}\ln N}{\pi^*(1-\lambda) N}})$$

% \label{theorem:hsu}
% \end{theorem}

% We can now use plug this estimator of the spectral gap inside the expression of $\gamma$.

% \begin{proposition}
% \label{proposition:lambda_est}
%     Let $\hat{\lambda}$ be defined as in Theorem \ref{theorem:hsu}. 

% Define the (asymptotic) estimator of $\gamma$ by

% $$\hat{\gamma}=\sqrt{\frac{\ln n(1-\hat{\lambda})}{n(1-\hat{\lambda})}}$$

% Then, for any $\delta\in[0,1]$

% $$\mathbb{P}_{D_{\textrm{tr}}}\bigg(|\hat{\gamma}-\gamma|= O_N(\frac{\hat{w}(N,\delta)}{(1-\lambda)}\gamma)\bigg) \geq 1-\delta$$ 

% \end{proposition}

% \subsection{Corrected split CP}

% Proposition \ref{proposition:cov_no_restart} provides us with a simple way to achieve $1-\alpha$ coverage by reducing the empirical quantile level to offset the presence of $\gamma$.

% \begin{remark}
%     Let $\gamma$ be as in proposition \ref{proposition:cov_no_restart}.
    
%     Define the following corrected quantile level

% $$\alpha'=\alpha-\gamma$$

% then 

% $$\mathbb{P}(Y_{n+1}\in C(X_{n+1}))\geq 1-\alpha$$
% \end{remark}  

% We state the same result but with the estimator of $\gamma$.
% \begin{proposition}
% \label{proposition:corollary_cov}
% For split CP with the corrected quantile level

% $$\alpha'=\alpha-\hat{\gamma}$$

% we have for any $\delta>0$ and $n$ large enough (such that the asymptotic expression of $\gamma$ holds)
% \begin{align*}
% \mathbb{P}(Y_{n+1}\in C(X_{n+1})) &\geq  (1-\alpha -O_N(\frac{\hat{w}(N,\delta)}{(1-\lambda)})\gamma)(1-\delta)   \\
% &\geq 1-\alpha-O_N(\frac{\hat{w}(N,\delta)}{(1-\lambda)})\gamma-\delta
% \end{align*}

% % \begin{itemize}[leftmargin=*]
% %     \item Consider a "worst case" scenario where we choose $\delta=0$. Then, with 
    
% %     $$\eta_0 = \frac{|\mathcal{X}|\min(|\mathcal{X}|,\ln \frac{1}{\pi^*})}{\pi^*(1-\lambda)^2}\sqrt{\frac{\ln\ln N}{\pi^*N}} $$
    
% %     we have

% %     $$\mathbb{P}(Y_{n+1}\in C(X_{n+1})) \geq  1-\alpha -\eta_0\gamma$$
    
% %     % \item Consider $\delta>0$ and let 
    
% %     % $$\eta=\sqrt{\frac{\ln N}{\pi^*(1-\lambda)^3 N}}$$

% %     % be the corresponding estimation error.
    
% %     % If $\eta\gamma>\sqrt{\frac{1}{e}}$ then the optimal value of $\delta$ is 0 and we return to the above case, else it is given by

% %     % $$\delta_{\textrm{min}}=|\mathcal{X}|\exp(\frac{1}{2}W_{-1}(-\frac{\eta^2\gamma^2}{2|\mathcal{X}|^2}))$$

% %     % Furthermore, for $\delta=\frac{|\mathcal{X}|\ln N}{\sqrt{N}}\gamma$, we obtain 
%     For $\delta=\frac{|\mathcal{X}|\ln N}{\sqrt{N}}\gamma$, and $\eta=\frac{\ln N}{\sqrt{\pi^*(1-\lambda)^3 N}}$ we obtain 
%     $$O_N(\frac{\hat{w}(N,\delta)}{(1-\lambda)})=O_N(\eta)$$

%     %Furthermore, let $u=\ln(\eta^2\gamma^2)$, we have the following interval 

%     %$$\exp(\frac{u}{2}-\sqrt{\frac{-u-1}{2}})\leq\frac{\delta}{|\mathcal{X}|}\leq \exp(\frac{u}{3}-\sqrt{\frac{-u-1}{2}}) $$

%     %Hence, for $N\rightarrow\infty, u\rightarrow -\infty$ and we have asymptotically

%     %$$\eta\gamma\leq\frac{\delta}{|\mathcal{X}|}\leq (\eta\gamma)^\frac{2}{3}$$

%     %which in turn gives the following asymptotic bound on the corollaryrected coverage gap
%     Hence,
%     \begin{align*}
%     &\mathbb{P}(Y_{n+1}\in C(X_{n+1})) \\
%     %&\geq  1-\alpha -\eta\gamma|\mathcal{X}|\sqrt{-\ln \eta\gamma} - (\eta\gamma)^\frac{2}{3}
%     &\geq 1-\alpha-O_N(\eta+\frac{|\mathcal{X}|\ln N}{\sqrt{N}})\gamma
%     \end{align*}
    
% \end{proposition}

% \begin{corollary}
% Denote by 

% $$\gamma_\textrm{corrected}=(\eta+\frac{|\mathcal{X}|\ln N}{\sqrt{N}})\gamma $$

% the coverage gap of corrected split CP. For $N$ large enough, we have 

% $$\gamma_\textrm{corrected}\leq \gamma$$

% \end{corollary} 
